Improved Surrogate Modeling using Machine Learning for Industrial Civil Aircraft Aerodynamics

Predicting and simulating aerodynamic fields for civil aircraft over wide flight envelopes represent a real challenge mainly due to significant numerical costs and complex flows. Surrogate models and reduced-order models help to estimate aerodynamic fields from a few well-selected simulations. However, their accuracy dramatically decreases when different physical regimes are involved. Therefore, a method of local non-intrusive reduced-order models using machine learning, called Local Decomposition Method, has been developed to mitigate this issue. This paper introduces several enhancements to this method and presents a complex application to an industrial-like three-dimensional aircraft configuration over a full flight envelope. The enhancements of the method cover several aspects: choosing the best number of models, estimating apriori errors, improving the adaptive sampling for parallel issues, and better handling the borders between local models. The application is supported by an analysis of the model behavior, with a focus on the machine learning methods and the local properties. The model achieves strong levels of accuracy, in particular with two sub-models: one for the subsonic regime and one for the transonic regime. These results highlight that local models and machine learning represent very promising solutions to deal with surrogate models for aerodynamics.

==> packages/toto.tex <==

%==============================================================
%                                                         PACKAGES
%==============================================================
% Fonts
%-----------
\usepackage	[english]{babel}		% typographie francaise
\usepackage{todonotes}
%\selectlanguage{french}			% typographie francaise
%\usepackage	[latin1]{inputenc}
%\usepackage[]{inputenc}   % pour taper les accents directement au clavier (pour MAC)
\usepackage[utf8]{inputenc}  % pour les accents
\usepackage[T1]{fontenc}                   % accents 
%\usepackage	{times}                  	% police "Times" (a changer en Euler pour les equations)
%\usepackage	{upgreek}			% pour avoir des lettres grecques droites
\usepackage[mathscr]{euscript}	% pour les lettres gothiques
\usepackage	{textcomp}		% symboles
\usepackage	{sectsty}			% pour changer la font des titres de section
\usepackage[Sonny]{fncychap} 	% pour changer la font des titres de chapitre. Choix entre les options : Sonny, Lenny, Glenn, Conny, Rejne, Bjarne
\usepackage	{Tabbing}			% pour faire des tabulations tout en inluant des caractères accentués
\usepackage{nameref}                        % Pour référencer des chapitres \nameref{chap:intro}

% Figures
%-----------
%\usepackage	{epsfig}			% pour inclure des images
\usepackage	{graphicx}			% pour inclure des images
%\usepackage	{psfrag}             		% pour remplacer des caracteres sur les .eps 
%\usepackage[absolute]{textpos}	%pour positionner des figures ou on veut
\usepackage[section]{placeins} % placement des figures

% Tableaux
%--------------
\usepackage	{array}
%\usepackage	{threeparttable}		% tables with footnotes
%\usepackage	{dcolumn}			% decimal-aligned tabular math columns
%\usepackage	{multirow}			% pour créer des tableaux avec des cases multicolonnes
%\usepackage	{multicol}
\usepackage{tabularx}
\usepackage{supertabular}
%\usepackage	{tabls}			% permet de gerer l'espacement vertical a l'interieur d'un tableau en ajoutant des commandes du type "[5pt]" ˆ l'interieur de \begin{tabular}
\usepackage{mdframed} % permet de faire les encadrer au debut de chapitre
\usepackage{makecell}

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
%\newcolumntype{C}{>{\centering\arraybackslash}X} 
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\newcommand\ch[1]{\centering                        % <--- added
    \begin{tabular}{@{}>{}c@{}}
                    #1
    \end{tabular}
                  }


% CaptionsR
%-------------
%\usepackage{ccaption}			% pour modif titre des Fig et des Tab
%\usepackage[geometry]{ifsym} 		% symbols for captions
%\usepackage[justification=centering]{caption}
\usepackage{caption}
%\usepackage{subfigure}
\usepackage{subcaption}

% Equations
%---------------
\usepackage{amsbsy,amscd}
\usepackage	{amsmath}
\usepackage	{amssymb}
\usepackage	{amsfonts}
%\usepackage	{mathptmx}		% change l'apparance de certains symboles mathematiques (non recommande)
\usepackage	{bm}				% bold math
\usepackage[chapter]{algorithm}
% Nice looking for empty set
\let\oldemptyset\emptyset
\let\emptyset\varnothing

\usepackage{algpseudocode}

\usepackage{dsfont} % pour pouvoir utiliser \mathds
\usepackage{siunitx} % pour pouvoir le symbole degree si

\newtheorem{hypothesis}{Hypothesis}{\bf}{\it}
\newtheorem{definition}{Definition}{\bf}{\it}
\newtheorem{proposition}{Proposition}{\bf}{\it}
\newtheorem{theorem}{Theorem}{\bf}{\it}
\newtheorem{remark}{Remark}{\bf}{\it}

% Colors
%----------
\usepackage	{color}	        				% pour personaliser les couleurs (RGB de 0 a 1)
\definecolor{lightgray}{gray}{0.66}
\definecolor{stronggray}{gray}{0.33}
\definecolor	{DarkBlue}{rgb}{0.0,0.0,0.0}	% definition de bleu sombre


% Hyperliens
%----------------
%\usepackage	[colorlinks=true,pagebackref=true,linkcolor=black,citecolor= darkblue,breaklinks]{hyperref}
\usepackage	[naturalnames=true,colorlinks=true,pagebackref=true,linkcolor=DarkBlue,citecolor= DarkBlue,breaklinks]{hyperref}
% Retirer colorlinks=true fait apparaitre les encadre de couleur
%\usepackage{xcolor}
%\usepackage	[pagebackref=true,linkcolor=DarkBlue,citecolor= DarkBlue]{hyperref}

% Glossaire
\usepackage{glossaries}
 \addto\extrasenglish{%
  \def\chapterautorefname{Chapter}%
}

% Bibliographie
%-------------------
%\def\backref{Cit\'e p.~}			%  facon dont apparait l'endroit ou sont citees les refs dans la biblio
%\usepackage[authoryear, square]{natbib}				% pour gerer le style des citations dans le texte
\usepackage[numbers, square]{natbib}

%\bibliographystyle{francais}

% Gestion des en-ttes et pieds de page
%----------------------------------------------------
%\usepackage{fancyheadings}	% pour avoir les titre des chap en haut de chaque page
\usepackage	{fancyhdr}			% pour les titre des chap en haut de page


% Autres
%-----------
%\usepackage	{pst-grad}   		% PSTricks related package for filling areas with a color gradient
%\newrgbcolor	{bgray}{0.9 0.9 0.9}
%\newrgbcolor	{bblue}{0.85 0.925 0.925}
\usepackage{cleveref}


% ==================
% Lors de l'importation du paquet, on doit lui passer comme option :
%   - Ets=<valeur> : permet de definir l'etablissement qui decerne le diplome
%   - ED=<valeur>  : permet de definir l'ecole doctorale et la specialite de la these
%   - ED2=<valeur> : permet de definir une deuxieme specialite. FACULTATIF.
% La liste des valeurs possibles pour ces deux options sont donnees respectivement dans
% les fichiers 'Ets-list.txt', 'ED-list.txt' et 'ED-list.txt'.
% Par exemple pour un diplome decerne par :
% Universit\'e Toulouse 3 Paul Sabatier (UT3 Paul Sabatier)
% on utilisera l'option Ets=UT3.
\usepackage[ED=MEGEP-DyF, Ets=INP]{tlsflyleaf} 
%\usepackage[ED=SDU2E-Ast, ED2=SDU2E-Eco, Ets=UT3]{tlsflyleaf}

\usepackage{tlsflyleaf} %PAge de garde univ toulouse


%\usepackage	[left=3cm,right=3cm,top=2cm,bottom=2.5cm,
%        			includehead,includefoot,headheight=15pt,verbose]{geometry}
			
\usepackage	{nomencl}			% nomenclature generation via makeindex
\usepackage	{ifthen}			% pour les catégories de la liste des symboles

%\usepackage	{verbatim}			% la commande "\verbatiminput" permet d'inclure un fichier en mode verbatim
%\usepackage	{moreverb}		% avec "\listinginput" et "\verbatimtabinput" permet d'inclure les documents en mode verbatim, avec ou sans numérotation des lignes

\usepackage{lscape}			% inserer une page en mode paysage

\usepackage	[final]{pdfpages}		% pour inclure des pdf



\usepackage{lscape}                              % pour les pages paysages
\usepackage{multirow}                          % multi-row

